CopyBench: Measuring Literal and Non-Literal Reproduction of Copyright-Protected Text in Language Model Generation

Evaluating the degree of reproduction of copyright-protected content by language models (LMs) is of significant interest to the AI and legal communities. Although both literal and non-literal similarities are considered by courts when assessing the degree of reproduction, prior research has focused only on literal similarities. To bridge this gap, we introduce CopyBench, a benchmark designed to measure both literal and non-literal copying in LM generations. Using copyrighted fiction books as text sources, we provide automatic evaluation protocols to assess literal and non-literal copying, balanced against the model utility in terms of the ability to recall facts from the copyrighted works and generate fluent completions. We find that, although literal copying is relatively rare, two types of non-literal copying -- event copying and character copying -- occur even in models as small as 7B parameters. Larger models demonstrate significantly more copying, with literal copying rates increasing from 0.2\% to 10.5\% and non-literal copying from 2.3\% to 5.9\% when comparing Llama3-8B and 70B models, respectively. We further evaluate the effectiveness of current strategies for mitigating copying and show that (1) training-time alignment can reduce literal copying but may increase non-literal copying, and (2) current inference-time mitigation methods primarily reduce literal but not non-literal copying.

==> outline.tex <==
% \section*{Paper Outline}

% tl;dr: We propose a benchmark to automatically quantify the factors that might infringement copyright in the language model output, and understand the effectiveness of the copyright mitigation approaches. 

% \begin{enumerate}
%     \item (Introduction)
%     \begin{enumerate}
%         \item Large language models are capable of memorizing and reproducing data seen during training. There are widespread discussions and legal cases concerning the risk of copyright infringement in language model outputs..
%         \item We aim to evaluate mitigation methods that protect copyrighted data while exploit the utilities of these data.
%         \item Contribution 1: We introduce the first evaluation pipeline for non-verbatim copying.
%         \item Contribution 2: We analyze the effectiveness of copyright risk mitigation on instruction-tuning models and decoding approaches.
%     \end{enumerate}
%     \item (Benchmark)
%     \begin{enumerate}
%         \item Overview: We analyze two types of copying in LM generation.
%         \begin{enumerate}
%             \item Previous studies mainly focused on the verbatim copying of copyrighted data.
%             \item Beyond verbatim copying, we also analyze cases where LMs reproduce content that is semantically similar to copyrighted data, but not necessarily verbatim identical.
%         \end{enumerate}
%         \item Verbatim Copying
%         \begin{enumerate}
%             \item (Copyright Protection: text completion task) We detect verbatim copying in the text completion task.
%             \item (Utility: short-form QA)  We analyze whether the model memorizes the knowledge in the tested corpus.
%         \end{enumerate}
%         \item Non-verbatim Copying
%         \begin{enumerate}
%             \item (Copyright Protection: creative writing task) In the context of creative writing, we detect how many reference events in the novel are included in the generated story.
%             \item (Utility: book summary QA) We analyze whether the model memorizes event-level knowledge of the tested novels.
%         \end{enumerate}
%     \end{enumerate}
%     \item (Analysis: mitigating by decoding methods)
%     \begin{enumerate}
%         \item Setup: Post-training can also be effective in preventing the generation of similar content. MemFree decoding can effectively reduce exact copying. Additionally, we explore how decoding parameters affect the copyright risk.
%         \item Claim 1: MemFree decoding significantly reduces verbatim copying but does not prevent non-verbatim copying.
%     \end{enumerate}
%     \item (Analysis: mitigating by alignment techniques)
%         \begin{enumerate}
%             \item Setup: Alignment techniques such as SFT and RLHF improve helpfulness while reducing harmfulness and hallucination. We aim to explore whether these techniques can be used for reducing copyright risks.
%             \item Claim 1: Alignment techniques are capable of reducing copyright risks while preserving the knowledge of the copyright-protected data.
%             \item Claim 2: Reducing verbatim copying does not necessarily reduce non-verbatim copying.
%         \end{enumerate}
%     \item (Two-side benchmark: How different prompts affect eliciting copyrighted contents?)
%     \begin{enumerate}
%         \item Setup: We aim to understand how different prompts affect the elicitation of copyrighted content and provide a test bed for constructing more adversarial prompts for future research. We evaluate both verbatim and non-verbatim copying in the book domain. For each test case, the ``title'', ``author'', and ``prefix'' are allowed to be used to construct prompts for the text completion task. We evaluate all prompts on the LLaMA-2-70B and LLaMA-2-70B-chat models.
%         \item Analysis: Is providing the title and author helpful? Is providing in-context demonstrations helpful?
%     \end{enumerate}
%     \item (Related Works)
% \end{enumerate}


==> tables/nonverbatim.tex <==
\begin{table}
\centering
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{1}{l}{}  & \multicolumn{5}{c}{Non-verbatim Copying}               
\\ \midrule

\multicolumn{1}{l}{} &
  \begin{tabular}[c]{@{}c@{}}Copying\\ (ER\textgreater{}=1, \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Copying\\ (ER\textgreater{}=5, \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Copying\\ (CR\textgreater{}=1, \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Copying\\ (CR\textgreater{}=3, \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Fluency\\ (5-scale)\end{tabular}

\\ \midrule

\textbf{LLaMA-2-70B}  & \textbf{38.3}        & \textbf{4.4}         & \textbf{27.2}        & \textbf{8.5}         & \textbf{2.90}        \\
LLaMA-2-70B-chat      & 33.3                 & 1.1                  & 13.2                 & 1.1                  & 4.20                 \\
Tulu-2-70B            & 43.4                 & 3.7                  & 32.1                 & 6.3                  & 3.69                 \\
Tulu-2-70B+DPO        & 47.1                 & 3.5                  & 30.3                 & 6.5                  & 4.11                 \\
w/ Sampling Decoding  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
w/ MemFree Decoding   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}

\\ \midrule

\textbf{LLaMA-2-13B}  & \textbf{27.0}        & \textbf{1.8}         & \textbf{16.4}        & \textbf{2.5}         & \textbf{2.27}        \\
LLaMA-2-13B-chat      & 24.0                 & 0.7                  & 10.4                 & 0.4                  & 4.24                 \\
Tulu-2-13B            & 30.2                 & 1.1                  & 17.8                 & 2.3                  & 3.61                 \\
Tulu-2-13B+DPO        & 35.4                 & 1.2                  & 19.6                 & 1.6                  & 3.99                 \\
Vicuna-13B-v1.5       & 25.9                 & 0.5                  & 10.2                 & 1.2                  & 4.23                 \\
w/ Sampling Decoding  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
w/ MemFree Decoding   & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}

\\ \midrule

\textbf{LLaMA-3-70B}  & \textbf{45.0}        & \textbf{5.6}         & \textbf{30.0}        & \textbf{10.2}        & \textbf{2.89}        \\
LLaMA-3-70B-instruct  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
\multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}


\\ \midrule

\textbf{Mixtral-7x8B} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{26.5}        & \textbf{6.2}         & \textbf{3.45}        \\
Mixtral-7x8B-Instruct & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \bottomrule
\end{tabular}%
% }
\caption{Non-verbatim copying in creative writing task.}
\label{tab:verb-align}
\end{table}


==> tables/prompts-results.tex <==

\begin{table*}[]
\centering
% \resizebox{0.9\textwidth}{!}{%
\small
\begin{tabular}{@{}l|r@{\hspace{0.5\tabcolsep}}>{\tiny}lr@{\hspace{0.5\tabcolsep}}>{\tiny}lr@{\hspace{0.5\tabcolsep}}>{\tiny}l|r@{\hspace{0.5\tabcolsep}}>{\tiny}lr@{\hspace{0.5\tabcolsep}}>{\tiny}l@{}}
\toprule
                              & \multicolumn{6}{c|}{Copying}                       & \multicolumn{4}{c}{Utility}   \\ \midrule
\multicolumn{1}{c|}{LMs} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Literal\\ (\%, ↓)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Events\\ (\%, ↓)\end{tabular}} &
  \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Characters\\ (\%, ↓)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Fluency \\ (Literal)\\ (↑)\end{tabular}} &
  \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}Fluency\\ (Non-literal)\\ (↑)\end{tabular}} \\ \midrule
\textbf{Llama2-70B}           & 2.0 &          & 4.4 &          & 8.5  &          & 2.72 &        & 2.90 &        \\
+ Completion Format           & 4.3 & (+117\%) & 8.6 & (+94\%)  & 16.4 & (+94\%)  & 2.72 & (0\%)  & 2.88 & (-1\%) \\ \midrule
\textbf{Llama2-70B + Tulu}    & 1.0 &          & 3.7 &          & 6.3  &          & 3.03 &        & 3.69 &        \\
+ Completion Format           & 0.7 & (-33\%)  & 3.7 & (-1\%)   & 5.2  & (-17\%)  & 2.79 & (-8\%) & 3.92 & (+6\%) \\ \midrule
\textbf{Llama2-70B + MemFree} & 0.0 &          & 3.3 &          & 7.9  &          & 2.63 &        & 2.90 &        \\
+ Completion Format           & 0.0 & (0\%)    & 8.6 & (+158\%) & 17.0 & (+116\%) & 2.76 & (+5\%) & 2.87 & (-1\%) \\
\bottomrule
\end{tabular}
% }
\caption{Copying scores for various prompt templates. Completion-style prompts elicit more copying behavior in pre-trained LMs but less in aligned LMs compared to dialogue-style prompts (default).
\pw{How are we getting a -1\% relative drop for Tulu completion format in events overlap if there are only 572 examples? 3.7\% of 572 is 21 examples so any change that (to 20 or 22 examples, say) would be a much larger than 1\% diff?}
}
\label{tab:prompts-results}
\end{table*}



==> tables/verbatim.tex <==
\begin{table}
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}ccccccc@{}}
\toprule
&
   &
  \multicolumn{5}{c}{Verbatim Copying}
  \\ \midrule
     &
  \begin{tabular}[c]{@{}c@{}}Copying \\ Copyrighted \\ (Avg. Rouge-L)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Copying\\ Copyrighted \\ (Rouge-L\textgreater0.8, \%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Copying \\ Public Domain \\ (Avg. Rouge-L)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}  Copying \\ Public Domain \\   (Rouge-L\textgreater 0.8, \%) \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Fluency \\ (5-scale)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Utilization of \\ Knowledge \\ (F1 Score)\end{tabular} 
\\ \midrule
\textbf{LLaMA-2-70B} &
  \multicolumn{1}{c}{\textbf{0.198}} &
  \textbf{2.0} &
  \textbf{0.379} &
  \textbf{19.3} &
  \textbf{2.72} &
  \textbf{0.197}
   \\
LLaMA-2-70B-chat &
  \multicolumn{1}{c}{0.157} &
  0.0 &
  0.157 &
  0.0 &
  3.69 &
  0.155 
   \\
Tulu-2-70B &
  \multicolumn{1}{c}{0.183} &
  1.0 &
  0.304 &
  10.7 &
  3.03 &
  0.192 
   \\
Tulu-2-70B+DPO &
  \multicolumn{1}{c}{0.177} &
  0.3 &
  0.272 &
  7.3 &
  3.31 &
  0.190 
   \\
w/ Sampling Decoding &
   0.191&
   2.3&
   0.327&
   14.0&
   2.72&
   /\\
w/ MemFree Decoding &
   0.181&
   0.0&
   0.379&
   19.3&
   1.97&
   0.197\\
w/ MemFree Decoding &
   0.181&
   0.0&
   0.245&
   0.8&
   1.97&
   0.197\\ \midrule
\textbf{LLaMA-2-13B} &
  \textbf{0.148} &
  \textbf{0.0} &
  \textbf{0.171} &
  \textbf{1.9} &
  \textbf{2.12} &
  \textbf{0.147} 
   \\
LLaMA-2-13B-chat &
  0.108 &
  0.0 &
  0.109 &
  0.0 &
  3.08 &
  0.128 
   \\
Tulu-2-13B &
  0.153 &
  0.0 &
  0.162 &
  0.0 &
  3.08 &
  0.139 
   \\
Tulu-2-13B+DPO &
  \multicolumn{1}{c}{0.157} &
  0.0 &
  0.161 &
  0.0 &
  3.43 &
  0.124 
   \\
Vicuna-13B-v1.5 &
  \multicolumn{1}{c}{0.151} &
  0.0 &
  0.155 &
  0.1 &
  3.77 &
  0.129 
   \\
w/ Sampling Decoding &
   &
   0.0&
   &
   1.3&
   &
   \\
w/ MemFree Decoding &
   &
   0.0&
   &
   1.9&
   &
   \\
w/ MemFree Decoding &
   &
   0.0&
   &
   0.0&
   &
   \\ \midrule
\textbf{LLaMA-3-70B} &
  \multicolumn{1}{c}{\textbf{0.279}} &
  \textbf{8.3} &
  \textbf{0.487} &
  \textbf{32.7} &
  \textbf{2.62} &
  \textbf{0.230} 
   \\
LLaMA-3-70B-instruct &
   &
   &
   &
   &
   &
   \\\midrule
\textbf{Mixtral-7x8B} &
  \multicolumn{1}{c}{\textbf{0.159}} &
  \textbf{0.7} &
  \textbf{0.212} &
  \textbf{4.9} &
  \textbf{2.85} &
  \textbf{0.154} 
   \\
Mixtral-7x8B-Instruct &
   &
   &
   &
   &
   &
   \\ \bottomrule
\end{tabular}%
}

    \caption{Performance of decoding techniques on copyright protection and utilization of knowledge in the copyrighted data. [The current figure is a placeholder]}
    \label{tab:verb-dec}
\end{table}

